Environmental dependence of polycyclic aromatic hydrocarbon emission at z~0.8. Investigation by observing the RX J0152.7-1357 with AKARI

We study the environmental dependence of the strength of polycyclic aromatic hydrocarbon (PAH) emission by AKARI observations of RX J0152.7-1357, a galaxy cluster at z=0.84. PAH emission reflects the physical conditions of galaxies and dominates 8 um luminosity (L8), which can directly be measured with the L15 band of AKARI. L8 to infrared luminosity (LIR) ratio is used as a tracer of the PAH strength. Both photometric and spectroscopic redshifts are applied to identify the cluster members. The L15-band-detected galaxies tend to reside in the outskirt of the cluster and have optically green colour, R-z'~ 1.2. We find no clear difference of the L8/LIR behaviour of galaxies in field and cluster environment. The L8/LIR of cluster galaxies decreases with specific-star-formation rate divided by that of main-sequence galaxies, and with LIR, consistent with the results for field galaxies. The relation between L8/LIR and LIR is between those at z=0 and z=2 in the literature. Our data also shows that starburst galaxies, which have lower L8/LIR than main-sequence, are located only in the outskirt of the cluster. All these findings extend previous studies, indicating that environment affects only the fraction of galaxy types and does not affect the L8/LIR behaviour of star-forming galaxies.

==> BK/data.tex <==
\section{Data and Methods}
In this study, we compare PAH behaviour of RXJ0152 with those of field environment in \cite{2014A&A...566A.136M}, who adopt $L8$ to LIR and $L8$ to $L4.5$ ratios as a tracer of PAH strength, and a ratio of LIR to $M_*$ as starburst strength, using AKARI north ecliptic pole deep survey \cite[hereafter NEP-Deep]{2006PASJ...58..673M,2008PASJ...60S.517W,2013A&A...559A.132M}.
We derive the same parameters for the RXJ0152 using {\it AKARI}/IRC, {\it Spitzer}/IRAC and MIPS, {\it Herschel}/PACS and SPIRE, and {\it Subaru}/S-cam.

\subsection{{\it AKARI}/IRC}
Twelve AKARI/IRC pointed observations were conducted at 2007 July 12-13 using S7 and L15 bands with AOT05 astronomical templates \cite[]{2007PASJ...59S.401O}.
The AOT05 performs no dithering nor filter change to obtain longer exposure time, where $\sim$30 sub-images with 16.4 seconds are taken.
The S7 and the L15 band images, whose field of views are separated by 20 arcmin, are taken simultaneously so that the alignment correction should be the same. 
The observations were consists of two fields, F1(28.1679,-13.9683) and F2 (28.3029,-13.9141).
The F1 field was observed four times with the L15 band and three times with the S7, and the F2 field was twice with the L15 and three times with the S7.
\par
The image reduction was performed on the basis of standard manner.
The linearity correction, dark subtraction, and flat fielding were done with the AKARI IRC imaging pipeline (version 131202).
Dark frame taken in each observation was used for the dark subtraction.
\par
The world coordinate system (WCS) information was registered into each sub-frame, using {\it Spitzer}/IRAC and MIPS image downloaded from the IRSA web site\footnote{http://irsa.ipac.caltech.edu/Missions/spitzer.html}.
Before registering the WCS information, we combined the sub-frames in each observation because there are not many stars in the S7 and little stars in the L15 images. 
The alignments of the L15 band is done with referring those of the S7 images, the same as \cite{2013A&A...559A.132M}. 
After registering the WCS information into the combined images, the WCS was copied into each sub-frame.
\par
Bad pixels were removed using the all-dark-frame-stacked images. 
A total of 72 dark images were stacked with median values for both S7 and L15 bands.
After removing the large scale gradient using median box car filter with 51-pixel size, pixels with outlier values were detected.
The outliers were determined as pixels whose values were above the 3$\sigma$ above the median value of the around 48 pixels, and pixels with masked by L.A.cosmic \cite[]{2001PASP..113.1420V} with default parameters.
We also masked the slit mask region for the S7 images and the X centre line (X=129) and a region [237:256,*] for the L15, since these regions may not have a regular response.
\par
The sky background of each images were subtracted after masking all sources that were detected in temporally stacked images to avoid influence of sources on the background estimation.
The source extraction was performed with SExtractor \cite[]{1996A&AS..117..393B}.
The SExtractor provides an image, in which only detected objects are remained, and this image was projected into each sub-frame and all source positions in each sub-frame were masked. 
%to know the pixel coordinates of the sources in each sub-frames.
We also used SExtractor to create a back ground map of each sub-frame and subtracted it from the sub-frames.
\par
After the sky background subtraction, all images were projected into a common image and combined with a 3 sigma clip.
The pixel sizes were reduced to 1 arcsec from 2.34$\times$2.34 and 2.51$\times$2.39 for S7 and L15, respectively.
In the stacking process, the image distortion was simultaneously corrected. 
The pixel values of the projected images were calculated with linear interpolation.
Fig.\ref{fig:L15map} shows the mosaicked L15 image, which covers a $\sim$ 10 $\times$ 20 arcmin$^2$) region.
The green broken circles indicates 2, 3, and 5 Mpc from the cluster centre, R.
The L15 image completely covers the region at $R<2$ Mpc. 
\begin{figure}
  \centering
  \includegraphics[width=90mm]{pictures/L15mapb.eps}
  \caption{Mosaicked L15 image ($\sim 10 \times 20$ arcmin$^2$).
    Blue square and magenta line indicate {\it Subaru/S-cam} and {\it Spitzer}/MIPS coverages.
    Green broken circles indicate 2, 3, and 5 Mpc radius from the cluster centre.
  \label{fig:L15map}}
\end{figure}
\par
Source extraction was performed on the mosaic images using SExtractor.
Sources with five connected pixels that are above 1$\sigma$ from the local background were detected.
Although this detection criteria was lose, which leads fake sources, they were removed from the final sample due to the matching with other catalogues.
\par
We applied aperture photometries on the detected sources with SExtractor.
Aperture radius was 6 arcsec, for which \cite{2013A&A...559A.132M} was estimated the photometric calibration.
The flux errors were estimated from the standard deviation of the sky background in the annulus of 20 arcsec with a 15 arcsec width.
Nonetheless, these errors should be underestimated because our mosaic image have a correlation between pixel values, due to the pixelation in the mosaicking.
To estimate how errors were underestimated, we also performed photometries at $\sim$400 random positions.
The standard deviation of the signal to noise ratio of the flux at the random position should lead the detection limit and a scaling factor, by which source flux errors should be multiplied.
The obtained scaling factors  were 3.85 and 3.70, and the detection limits were 76 and 268 $\mu$Jy for S7 and L15 bands, respectively.
These scaling factors were quite larger than expected from the pixelation, which are 2.34 and 2.45.
A possible explanation is that the random-sky-flux distribution contains sky gradient in the images, which may not be removed from the sky subtraction. 
Hence, we may overestimate the source-flux errors, but we apply these errors as conservative errors.

%\subsection{{\it Spitzer} and {\it Herschel}}
\subsection{{\it Spitzer}/IRAC and MIPS}
We retrieved the {\it Spitzer} data from the IRSA website.
All PBCD data around the cluster was downloaded for both IRAC and MIPS. 
Sky background was subtracted from each image using a median filtered image after masking the sources.
The box sizes of the median filter are 51 and 31 pixels for IRAC 1-4 channels and MIPS 24 $\mu$m band.
The smaller box size was applied for the MIPS because it showed strong residual of the sky background in PBCD images.
After the sky subtraction, all images were aligned and combined with median values.
The magenta line in Fig.\ref{fig:L15map} shows the coverage map of the MIPS image, which completely covers the region at $R<$ 3 Mpc.
The IRAC image also covers $R\ltsim$ 3 Mpc, although it is not shown in the figure for simplicity.
%\color{red}{largaer than marcillac. typical exposure time 2ks. deviation?}
%\color{black}
\par
Source extractions were performed using SExtractor. 
Sources with five connected pixels above 1$\sigma$ from the background were extracted. 
Similar to {\it AKARI} sources, fake sources were contained, which removed from the matching with other catalogues. 
Photometries were simultaneously done for IRAC 1-4 channels with the dual mode of the SExtractor, where we used the [3.6] band image as the detection image and aperture radius was set to 6 arcsec.
Photometries for MIPS 24 $\mu$m band were done with 7 arcsec aperture radius and sky background was estimated from the annulus of 15 arcsec with a 5 arcsec width, because the residual background was strong even after the subtraction of the median filtered image and hence the local sky background should be estimated from regions as near from the sources as possible. 
The flux errors were also estimated from the sky background around the sources for both IRAC and MIPS, because errors output from SExtractor are not estimated from the region around sources.
The region of the sky background for IRAC images was a annulus of 14.4 arcsec with 9.6 arcsec width. 
Considering the correlation between pixel values, we scaled the errors with the same methods as the {\it AKARI} sources. 
The scaling factors were 3.17, 2.96, 2.92, 2.82, 2.69 for IRAC 1-4 channels and MIPS24. 
Similar to {\it AKARI} sources, although these factors maybe over estimated, we applied these values as conservative values.
\par
\subsection{{\it Herschel}/PACS and SPIRE}
{\it Herschel} observed the RXJ0152 with PACS and SPIRE as Evolutionary Probe (PEP) \cite[]{2011A&A...532A..90L}, and the catalogue of 100 and 160 $\mu$m bands of the PACS and 250, 350, and 500 $\mu$m bands of the SPIRE are available.
We downloaded all these catalogues from the CDS. 
Although it is also observed with SPIRE as Herschel Multi-tiered Extragalactic Survey \cite[]{2012MNRAS.424.1614O}, we did not use these data for simplicity.

\subsection{{\it Subaru}/Suprime-Cam}
{\it Subaru}/S-cam $V R i' z'$ images were obtained in \cite{2005PASJ...57..309K}.
The reduction procedure is described in \cite{2005PASJ...57..309K}.
The detection limits of these bands with 2 arcsec aperture were reported as 26.7, 26.5, 26.1 and 25.0, for $V$, $R$, $i'$ and $z'$ bands, respectively.
The coverage is shown in Fig.\ref{fig:L15map} with a blue square.
Source extraction was also done using SExtractor and objects with 5 connected pixels whose values were more than 1.5$\sigma$ above the background were detected.
This detection criteria is with default parameters of the SExtractor.
Photometries were performed with the dual mode using the $z'$ band image as a detection image and $MAG\_AUTO$ was applied for measuring the total magnitudes.
We added 0.05 magnitude errors for uncertainty of magnitude zero points for all bands. 

\subsection{Matching the catalogues}
To merge the above catalogues, sources were cross-matched with the nearest neighbour method. 
{\it Subaru} sources were matched with {\it Spitzer}/IRAC sources with a 1 arcsec search radius.
IRAC sources were matched with AKARI/S7, L15 and MIPS24 sources with 2.5 arcsec radii, respectively, where the size of the 2.5 arcsec search radius is the same as the matching in \cite{2013A&A...559A.132M}.
Finally, {\it Herschel}/PACS and SPIRE sources were matched with MIPS24 sources with 5 and 6 arcsec radii, which are the same as in \cite{2014A&A...566A.136M}.
We used only objects that have both IRAC and {\it Subaru} photometries to avoid fake sources and to make photometric redshifts reliable.
\par
We also matched these sources with spectroscopically confirmed members provided by many researchers \cite[]{2005A&A...432..381D,2010ApJ...725.1252D,2005AJ....129.1249J,2006MNRAS.365.1392T}.
%We note that galaxies provided by \cite{2006ApJ...644...30B} are from \cite{2005A&A...432..381D} 
All these sources were matched with {\it Subaru} sources with a 1 arcsec search radius. 
In the matching process, we had a problem that the coordinates of a part of the sample from \cite{2005A&A...432..381D} was out of the position, although the sample listed in \cite{2006ApJ...644...30B}, which are from \cite{2005A&A...432..381D}, is located at the right position.
Hence, we used sample from \cite{2006ApJ...644...30B} instead of \cite{2005A&A...432..381D}, although the former has no spectroscopic redshift information.
The redshift of these members were assumed to be $z$=0.84.
Assuming objects with $z_{spec}$=0.81-0.87 are member galaxies, a total of 186 spectroscopically confirmed members were obtained, among which 30 objects were detected with the {\it AKARI} L15 band.
We note that some member objects were rejected due to lack of IRAC photometries.

\subsection{Photometric redshifts}
The photometric redshifts were calculated using a publicly available software, LePHARE \cite[]{2006A&A...457..841I,2007A&A...476..137A}. 
It performs a template fitting with the spectral energy distribution (SED) for each object, and calculates photometric redshift as well as physical parameters, with which minimum $\chi^2$ is provided.
\par
We used AVEROIN SED templates \cite[]{2007A&A...476..137A} with an interstellar extinction law of SMC.
The {\it Subaru}/S-cam $VRi'z'$ to IRAC [3.6] and [4.5] were fitted with the templates, where [3.6] and [4.5] covers longer wavelength than a stellar bump at 1.6 $\mu$m. 
We applied the ``AUTO\_ADOPT'' option, which calculates photometric zero point correction to minimise the difference between SEDs of objects with spectroscopic redshift and best fit templates. 
\par
The accuracy of the photometric redshifts was calculated with spectroscopic redshifts. 
Figure \ref{fig:zpzs} shows the distribution of the difference of photometric and spectroscopic redshifts for the 186 member galaxies.
The average after 3$\sigma$ clips is $z_{phot}-z_{spec}$ = -0.0038 and the standard deviation is $\sigma_{zp}$ = 0.080, which corresponds to $\delta z_{phot}/(1+z_{spec})$=0.044.
Ten galaxies have outlier $z_{phot}$ and were clipped in the calculation. 
The $z_{phot}$ distribution for the member galaxies are $z_{phot}$=0.843$\pm$0.0825 so that we assumed that objects with $z_{phot}$=0.76-0.925 are cluster member galaxies.
In total, 1922 galaxies were identified as member galaxies, among which 122 have  MIPS photometry. 
We visually checked the SED of these MIPS detected sources, and found no galaxies with an unusual SED.
Among the total sample, 333 galaxies were located in the $R<$ 2 Mpc region. 
\begin{figure}
  \includegraphics[angle=270,width=80mm]{pictures/zpzs.ps}
  \caption{Distribution of $z_{phot}-z_{spec}$ for 186 member galaxies.
  The standard deviation is $\sim$0.08.
%  Among 186 galaxies, 10 members have outlier values (3$\sigma$) 
  \label{fig:zpzs}}
\end{figure}

\subsection{Deriving physical parameters with SED fitting}
The main purpose of this paper is to compare behaviour of the 8$\mu$m luminosity of cluster and field galaxies, which was investigated in \cite{2014A&A...566A.136M}.
Since they used physical parameters of LIR, $M_*$, $L8$ and $L4.5$ calculated with the LePHARE, we also derive these parameters with similar methods.
\par
Infrared luminosities LIR, integrated over 8$\mu$m to 1000$\mu$m, were estimated with 24 $\mu$m to 500 $\mu$m photometries.
We did not use L15 photometries because it was used to derived $L8$ and to avoid any dependency between $L8$ and LIR. 
An SED library of \cite{2001ApJ...556..562C} was used for the calculation.
For a total of 122 galaxies, among which 22 have $Herschel$ photometries, LIR were derived. 
%magerr<1. >1を含めると145
Although most of the LIR were derived with only 24 $\mu$m luminosity, they can be reliable since \cite{2010A&A...518L..29E} shows infrared luminosities derived from only 24 $\mu$m band agree with those from 24 $\mu$m and 100-500 $\mu$m bands within 0.15 dex for galaxies at $z<$1.5.
\par
Stellar masses $M_*$ were derived with $VRi'z'$, [3.6] and [4.5] photometries using an SED library of BC03 \cite[]{2003MNRAS.344.1000B}.
Since these six bands cover the below and above 4000$\AA$ breaks, $M_*$ can be reliably determined. 
We adopted SEDs of solar metallicity with $\tau$ of 0.1-10 Gyr and an extinction law of \cite{2000ApJ...533..682C}.
The $AUTO\_ADOPT$ option was also applied.
To check whether we can see the star-formation main sequence, we plot the infrared luminosities, which correspond to SFR, and stellar mass, in Fig.\ref{fig:ms}.
\begin{figure}
  \includegraphics[width=60mm,angle=270]{pictures/ms.ps}
  \caption{Infrared luminosity versus stellar mass.
    Black solid line and grey broken lines indicate the best fit for star-forming galaxies and the scatter of each point.
    Grey dotted line indicates the border line which separate passive and star-forming galaxies.
  \label{fig:ms}}
\end{figure}
We can see a relation between them.
The best fit line without using galaxies below 0.6 log $M_*$+4.5 line (grey dotted line in the figure) is log LIR = 0.36 log $M_*$+7.5, and the scatter is 0.20 dex.
Hereafter we call galaxies below 0.6 log $M_*$+4.5 line passive and those above line star-forming galaxies.
\par
$L8$ and $L4.5$ were derived with less uncertainty from $K$-correction using L15 and IRAC4 bands.
This is because 8 and 4.5 $\mu$m band is redshifted into L15 and IRAC4 bands at $z\sim0.8$. 
The $K$-correction was estimated with 25 SED templates from \cite{2006ApJ...642..673P,2007ApJ...663...81P}. 
The IRAC2 and IRAC4 bands were used for 4.5 and 8 $\mu$m bands for the $K$-correction. 


